Mapping the Spiral of Silence: Surveying Unspoken Opinions in Online Communities

We often treat social media as a lens onto society. How might that lens distort the popularity of political and social viewpoints? We examine discrepancies between publicly posted and privately surveyed opinions within communities, contributing a measurement of the "spiral of silence" theory; the theory posits people are less likely to voice opinions when they believe they hold minority views, creating a reinforcing cycle where these opinions are expressed less. We surveyed members of politically-oriented Reddit communities about their willingness to post on contentious topics, yielding 439 responses across twelve subreddits. 72.1% of participants who perceive themselves in the minority remain silent and are half as likely to post compared to those who believe their opinion is in the majority. Community design factors, such as perceived diversity, are associated with less self-silencing. We provide recommendations for counteracting self-silencing at the community level (e.g., positive reinforcement, more transparent moderation). Overall, these results reveal gaps between online discourse and broader public opinion.

==> Tables/avoid_table.tex <==
\begin{table}[htbp!]
    \centering
    \caption{Summary of actions that participants reported that they would take if they did not feel comfortable sharing a viewpoint, meaning they agreed with a viewpoint but reported that they were unlikely to share the opinion to a given subreddit.}
    \begin{tabular}{lr}
    \toprule
    \textbf{Action} &  \textbf{N}\\
    \midrule
    Read discussion on a topic but not share viewpoint & 68 \\
    Discuss with friends and family offline & 34 \\
    Choose to ignore discussion on topic & 19 \\
    Post viewpoint using a throwaway account & 11 \\
    Post to a different subreddit & 3 \\
    Other & 3 \\
    \bottomrule
    \end{tabular}
    \label{tab:otheractions}
\end{table}

==> Tables/subreddits.tex <==
\begin{table}[ht!]
    \small
    \centering
    \caption{List of subreddits included in our analysis, the number of viewpoints collected for each subreddit, and political leaning of the community. The partisanship ratings come from \citet{waller2021quantifying} community embeddings. Four of the subreddits did not have partisanship ratings (marked as ``NA'').}
    \begin{tabular}{lrr}
    \toprule
    Subreddit &  \# of Viewpoints & Partisanship\\
    \midrule
    againsthatesubreddits & 1 & Left\\
    anarchy101 & 5 & Center\\
    askfeminists & 1 & Center\\
    austrianeconomics & 1 & Right\\
    canada & 2 & Right-Center\\
    changemyview & 56 & Center\\
    combatfootage & 14 & Right-Center\\
    conservative & 60 & Right\\
    conspiracy & 45 & Right Center\\
    economics & 30& Center\\
    europe & 2& Center\\
    feminism & 26& Left Center\\
    geopolitics & 7& Center\\
    latestagecapitalism & 29& Left\\
    law & 12& Center\\
    libsofreddit & 4&NA\\
    mensrights & 4& Right Center\\
    moderatepolitics & 3& Center\\
    news & 7& Center\\
    politicalcompassmemes & 1& NA\\
    politics & 147 & Left Center\\
    propagandaposters & 5 & Left Center\\
    qultheadquarters & 1 & NA\\
    redscarepod & 3 & NA\\
    sandersforpresident & 3 & Left\\
    socialism & 21 & Left\\
    subredditdrama & 10 & Left\\
    trump & 3 & Right Center\\
    twoxchromosomes & 1 & Left Center\\
    unitedkingdom & 1 & Center\\
    vaxxhappened & 5 & Left Center\\
    worldnews & 116 & Center\\
    youshouldknow & 1 & Center\\
    \bottomrule
    \end{tabular}
    \label{tab:subreddits}
\end{table}
